Exploring the Dynamics of Mass Action Systems

We present the Populus toolkit for exploring the dynamics of mass action systems under different assumptions.

==> eptcsdata.tex <==
\providecommand{\firstpage}{84}
\providecommand{\publicationstatus}{T. Dang and C. Piazza (Eds.): HSB 2013\\
EPTCS 125, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.125.6}{10.4204/EPTCS.125.6}}
\pdfoutput=1

